Fact-Checking the Output of Large Language Models via Token-Level Uncertainty Quantification

Large language models (LLMs) are notorious for hallucinating, i.e., producing erroneous claims in their output. Such hallucinations can be dangerous, as occasional factual inaccuracies in the generated text might be obscured by the rest of the output being generally factually correct, making it extremely hard for the users to spot them. Current services that leverage LLMs usually do not provide any means for detecting unreliable generations. Here, we aim to bridge this gap. In particular, we propose a novel fact-checking and hallucination detection pipeline based on token-level uncertainty quantification. Uncertainty scores leverage information encapsulated in the output of a neural network or its layers to detect unreliable predictions, and we show that they can be used to fact-check the atomic claims in the LLM output. Moreover, we present a novel token-level uncertainty quantification method that removes the impact of uncertainty about what claim to generate on the current step and what surface form to use. Our method Claim Conditioned Probability (CCP) measures only the uncertainty of a particular claim value expressed by the model. Experiments on the task of biography generation demonstrate strong improvements for CCP compared to the baselines for seven LLMs and four languages. Human evaluation reveals that the fact-checking pipeline based on uncertainty quantification is competitive with a fact-checking tool that leverages external knowledge.

==> tex/img/bio-example-FM-t.tex <==
\setlength{\columnsep}{0.3pc}

\begin{figure*}[h]
	\centering
	\scriptsize
 \begin{multicols}{2}

Maximum Probability
 
	\begin{tcolorbox}[size=fbox,
		title=\,{\includegraphics[width=1.5em]{tex/img/user-icon.png}\,\,\,Tell me a bio of Freddie Mercury.},
		colback=gray!2!white,
		colframe=cyan!15!white,
            coltitle=black,
		width=32em,
		sharp corners=northwest,
		]
			\includegraphics[width=1.5em]{tex/img/llm-icon.png}
			 \,\,\,Freddie Mercury was a British singer, songwriter, and pianist, best known as the lead vocalist of the rock band Queen. He was born on September 5, 1946, in Tanzania, East Africa, to parents of Indian and Iranian descent. He began his music career in the 1960s, performing with various bands in London before joining Queen in 1970. \newline
		
			Mercury was known for his \marktext{myorange}{powerful voice} and \marktext{myorange}{flamboyant stage presence}, and he wrote many of Queen's hit songs, including "Bohemian Rhapsody," "Killer Queen," and "We Are the Champions."  ...

	\end{tcolorbox}

\columnbreak

Claim-Conditioned Probability (ours)

\begin{tcolorbox}[size=fbox,
		title=\,{\includegraphics[width=1.5em]{tex/img/user-icon.png}\,\,\,Tell me a bio of Freddie Mercury.},
		colback=gray!2!white,
		colframe=cyan!15!white,
            coltitle=black,
		width=32em,
		sharp corners=northwest,
		]
			\includegraphics[width=1.5em]{tex/img/llm-icon.png}
			\,\,\,Freddie Mercury was a British singer, songwriter, and pianist, best known as the lead vocalist of the rock band Queen. He was born on September 5, 1946, in Tanzania, East Africa, to \marktext{myorange}{parents of Indian and Iranian descent.} He began his music career in the 1960s, performing with various bands in London before joining Queen in 1970. \newline
		
			Mercury was known for his powerful voice and flamboyant stage presence, and he wrote many of Queen's hit songs, including "Bohemian Rhapsody," "Killer Queen," and "We Are the Champions."  ...
	\end{tcolorbox}
 
 \end{multicols}
	    \caption{Visual comparison of our proposed Claim-Conditioned Probability method to the Maximum Probability baseline. CCP accurately identifies the incorrectly specified descent (in \colorbox{myorange}{red}),  whereas Maximum Probability erroneously emphasizes claims that are actually correct.}
	\label{fig:token-level_comparison}
\end{figure*}

